An Alloy Verification Model for Consensus-Based Auction Protocols

Max Consensus-based Auction (MCA) protocols are an elegant approach to establish conflict-free distributed allocations in a wide range of network utility maximization problems. A set of agents independently bid on a set of items, and exchange their bids with their first hop-neighbors for a distributed (max-consensus) winner determination. The use of MCA protocols was proposed, $e.g.$, to solve the task allocation problem for a fleet of unmanned aerial vehicles, in smart grids, or in distributed virtual network management applications. Misconfigured or malicious agents participating in a MCA, or an incorrect instantiation of policies can lead to oscillations of the protocol, causing, $e.g.$, Service Level Agreement (SLA) violations. In this paper, we propose a formal, machine-readable, Max-Consensus Auction model, encoded in the Alloy lightweight modeling language. The model consists of a network of agents applying the MCA mechanisms, instantiated with potentially different policies, and a set of predicates to analyze its convergence properties. We were able to verify that MCA is not resilient against rebidding attacks, and that the protocol fails (to achieve a conflict-free resource allocation) for some specific combinations of policies. Our model can be used to verify, with a "push-button" analysis, the convergence of the MCA mechanism to a conflict-free allocation of a wide range of policy instantiations.

==> challenges.tex <==
%The key to good modeling is abstraction.
%Our first effort of modeling the consensus-based auction protocol led into a detailed model.
%
% motivation going straight to the point (message)
In this section we analyze the performance of our model, when asserting the consensus property across different models of the same protocol. Our aims are to  demonstrate the design challenges of Alloy, and motivate the need for a careful abstraction choice. 

Alloy models encoded with suboptimal abstractions scale poorly. For example, the Alloy Analyzer run for $23$ hours to check the \texttt{consensus}  assertion  for the model we have presented, with a scope of merely $3$ physical nodes, $2$ virtual nodes and $12$ states~\footnote{All our experiments were carried out on a Linux machine running Intel core i3 CPU at 1.4GHz and 4 GB of memory.}
 Alloy cannot leverage parallelization, and its running time is dominated by the number of primary variables and clauses generated by the Analyzer.

%In Alloy the SAT instance result from checking any assertion is composed of a specific number of clauses and primary variables. 

%Simplifying complicated facts and combine facts 

%In the first try to improve the model, we tried to combine those facts that infer each other and simplified the complicated ones.

The conflict resolution table of the asynchronous max-consensus auction protocol has over $30$ complex predicates that regulates the actions that receiving agents should take upon reception of a bid message.
%
These rules are encoded in the \texttt{messageProcessing} predicate, that alone 
generated over $259,000$ SAT clauses. 
By combining logical statements, we compacted the set of rules to 12, reducing the number of number of SAT clauses to about $190,000$.

%For instance the major complication in our model is in the implementation of the \texttt{messageProcessing} predicate. This predicate models the rules of the table for conflict resolution in the consensus-based auction protocol. Each row of this table determines the action of the agents (physical nodes) upon receiving a new message.
%We manage to combine many of these rules (31 rules of the table could be compacted into only 12 rules).
%These set of simplifications helped us to reduce the number of clause in the SAT  problem from 259845 to 190974.


The model presented in Section~\ref{sec:VNE-model} uses integer variables and ternary relations when defining the three signatures \texttt{pnode}, \texttt{bidVector} and \texttt{message}.
Ternary relations and integers are convenient, as they  directly refer to the vectors  ${\bf a}$, ${\bf b}$, ${\bf t}$, defined in Section~\ref{sec:problem}, but lead to inefficiency of the Alloy Analyzer.

% but not efficient regarding the running time of the Alloy Analyzer. Hence in our final model, ternary relations are modeled using binary relations and also an abstract model for integers is used.


%we can re add this details later, but maybe not in this section. Here we only have to discuss the performance evaluation.
%
Modeling each ternary relation with two binary relations, we were able to reduce the number of primary variables from $990$ to $502$ variables, speeding up the performance of the Alloy Analyzer.
%
\texttt{bidTriple} is an example of signature converted to use solely binary relations:
%
%
{\scriptsize
\begin{verbatim}
    sig bidTriple{
        bid_v: one vnode,
        bid_b: one Int,
        bid_t: one Int,
        bid_w: one (pnode + NULL)
    }
\end{verbatim}
}
%
\junk{
Each instance of signature \texttt{bidTriple} corresponds
to every auctionable item (virtual node) one agent (physical node) as the winner (modeled by $\texttt{bidTriple\_w}$),
one bid value (modeled by $\texttt{bidTriple\_b}$) and a time stamp (modeled by $\texttt{bidTriple\_t}$).
For example, using this new signature the definition of signature $\texttt{message}$ looks like the following:
%
{\scriptsize
\begin{verbatim}
    sig message{
        msgSender: one pnode,
        msgReceiver: one pnode,
        msgBidTriples: set bidTriple
    }
\end{verbatim}
}
}
%
%Applying this set of changes in our model, reduced the number of primary variables from $990$ variables to $502$ variables.
%It is worth to mention that
%in all these comparisons the same scope is used and the same assertion (namely \texttt{consensus}) is checked.

%Yet the new model is far from perfect model.
%The current model uses the integer values and many binary integer operators.
%The use of integer values is in contradiction with having a good abstraction.
%As in ``Software Abstraction" \cite{} by Daniel Jackson,
%in discussion on integers, the author asserts that ``Integers are actually not very useful. If you think you need them, think
%again!" and also it is mentioned that Alloy is not a suitable tool for modeling a problem with
%heavy use of integers.
%Hence we implemented our own abstract model of numbers in module \texttt{valueModule} using signature \texttt{value}:
The Alloy's predefined integer (signature \texttt{Int}) can also be abstracted away using a new model of numbers in module \texttt{valueModule} defined by signature \texttt{value}:

%
{\scriptsize
\begin{verbatim}
    sig value{
        succ: set value,
        pre: set value
    }
\end{verbatim}
}
%

%In our model of numbers we don't care about the value of each instance of the \texttt{value}.
%In this model, the value of instances of numbers is not considered.
Each instance of signature \texttt{value} represent a number, But these instances does not
have any numerical value (for example the object ''\texttt{3}" representing the number three, has value $3$).
In module \texttt{valueModule} and \texttt{value} we only models relations between numbers. Using two relations \texttt{succ} and \texttt{pre}
we modeled binary operators $<$, $\leq$, $>$ and $\geq$ respectively using binary predicates \texttt{valL[,]},
\texttt{valLE[,]}, \texttt{valG[,]} and \texttt{valGE[,]}. For example for two instances \texttt{v1} and \texttt{v2}
of signature \texttt{value},
we have \texttt{v1} $\leq$ \texttt{v2} if predicate \texttt{valLE[v1, v2]} is true (which in our Alloy model is equivalent to say \texttt{v1 in v2.pre}).

In the new model, for the same scope as before, we managed to reduce the number of variables
from 502 to 446 and the number of clauses from 190974 to 114648.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to show the effect of good abstraction,
the performance of the Alloy Analyzer is investigated in two cases, the case using Alloy's predefined integer, in contrast to the case of using
\texttt{valueModule}.
All experiments were carried out on a personal computer powered by
 Intel core i3 CPU @ 1.4GHz with 4 GB of memory.
For each case we did ten experiments and the average of running time was recorded. The same search scope were used in both cases (three agents, two items and twelve states).
\junk{
Each experiment contains checking two assertions,
\texttt{consensus} and \texttt{numOfState}. The assertion \texttt{numOfState} asserts that there
exist some scenarios that our system, modeled as a ``state transition system",
passes through \texttt{val} number of states.%, which means \texttt{val-1} number of messages are being processed.
The other assertion \texttt{consensus} asserts that in all those scenarios after \texttt{val}$^{th}$
state the network reach consensus.
}

The running time and result of checking the consensus assertion for each case is presented in Table \ref{tab-comparison}.

\begin{table}[h]
\footnotesize
\caption{Performance analysis in different modeling approaches} % title name of the table
%\centering % centering table
\begin{tabular}{ p{1.1cm} p{0.6cm} | p{2.6cm} | p{2.6cm} } % creating 4 columns
\hline\hline % inserting double-line
  Assertion & &Case 1: Using Int & Case 2: Using value
\\[0.5ex]
\hline
 & result & No counterExpl found &  No counterExpl found \\[-1ex]
 \raisebox{1.5ex}{consensus}
 & time & 362.3 sec & 109.3 sec \\ [-1ex]
\hline % inserts single-line
\end{tabular}
\label{tab-comparison}
\end{table}

%
%
\junk{
\begin{table}[h]
\footnotesize
\caption{Performance analysis in different modeling approaches} % title name of the table
%\centering % centering table
\begin{tabular}{ p{1.1cm} p{0.6cm} | p{2.6cm} | p{2.6cm} } % creating 4 columns
\hline\hline % inserting double-line
  Assertion & &Case 1: Using Int & Case 2: Using value
\\[0.5ex]
\hline
 & result & No counterExpl found &  No counterExpl found \\[-1ex]
 \raisebox{1.5ex}{consensus}
 & time & 362.3 sec & 109.3 sec \\ [-1ex]
 \hline
 & result & counterExpl found &  counterExpl found \\[-1ex]
 \raisebox{1.5ex}{numOfState}
 & time & 4.4 sec & 4.0 sec \\[-1ex]
% [1ex] adds vertical space
\hline % inserts single-line
\end{tabular}
\label{tab-comparison}
\end{table}
}


==> open-question.tex <==
{\bf Path bidding}: how does the model change with path bidding instead of node bidding only?

==> protocol.tex <==
%\section{Problem Definition}\label{sec:problem}
%\vspace{-0.05in}






Consider a VNET embedding request by an SP (Figure~\ref{fig:VNexample}a) on a physical network (Figure~\ref{fig:VNexample}b) where each physical node (PN) belongs to a different InP. The SP sends to (a subset of) all physical nodes a request with (a subset of) the virtual elements (nodes and links), $e.g.$ virtual nodes VN1 and VN2 connected by virtual link VL1. Each physical node $i$, where $i \in V_G$, uses a private utility function $\mathbf{U}_i \in \mathbb{R}_{+}^{|V_H|}$  to bid on the virtual nodes, knowing that it could be the winner of a subset (for example VN1 or VN2 or both), and stores its bids in a vector $\mathbf{b}_i \in \mathbb{R}_{+}^{|V_H|}$. Each entry $b_{ij} \in \mathbf{b}_i$  is a positive real number representing the highest bid known so far on virtual node $j \in V_H$.
%
Also, physical nodes store the identifiers of the virtual nodes on which they are bidding in a list (bundle vector) $\mathbf{m}_i \in V_H^{T_{i}}$, where  $T_{i}$ is a target number of virtual nodes mappable on $i$. After the private bidding phase, each physical node exchanges the bids with its neighbors, updating  an assignment vector $\mathbf{a}_i \in V_G^{|V_H|}$ with the latest information on the current assignment of all virtual nodes, for a distributed auction winner determination.

%
The winner physical nodes communicate the mapping to the SP which, if possible, releases the next VNET(s) or the next VNET partition if any ($e.g.$ VN3, VN4, VL3 in Figure~\ref{fig:VNexample}$a$)~\footnote{The VNET partitioning problem has been shown to be NP-hard, $e.g$ in~\cite{Houidi2011} and it is outside the scope of this paper.}.
 %
 %
 Once the physical nodes have reached consensus on who is the winner for all the  virtual nodes of the (partial or full) VNET released for the auction, a distributed link embedding phase is run to embed each virtual link on a set of (one or many) loop-free physical paths (Figure~\ref{fig:VNexample}c.)
 %
 The mechanism iterates  over multiple node bidding and agreement (consensus) phases asynchronously, that is, the second bidding phase can start even if the first agreement phase is not terminated. Physical nodes act upon messages received at different times during each bidding phase and each consensus phase; therefore, each individual phase is also asynchronous. In the rest of the paper, we denote such {\it rounds or iterations} of node bidding followed by consensus with the letter $t$ and we omit $t$ when it is clear from the context.
 %

Adapting the definition of {\it max-consensus} from the consensus literature~\cite{consensusBook} to the VNET embedding problem we have:
%
\begin{definition}\label{def:maxConsensus}({\it max-consensus}.)
Given a physical network $G$, an initial bid vector of physical nodes  $\mathbf{b}(0) \stackrel{\Delta}{=} (\mathbf{b}_1(0), \ldots, \mathbf{b}_{|V_G|}(0))^{\rm T}$, a set of neighbors $\mathcal{N}_i \; \forall  i \in V_G$,  and the consensus algorithm for the communication instance $t+1$:
\begin{equation}
\mathbf{b}_i(t+1) = \max_{j \in \mathcal{N}_i  \cup \{ i \} }\{\mathbf{b}_j(t)\} \;\; \forall i \in V_G,
\end{equation}
\emph{Max-consensus} on the bids among the physical nodes is said to be achieved with convergence time $\tau$, if $\exists \; \tau \in \mathbb{N}$ such that $\forall \; t \geq \tau$ and $\forall \; i, i^{\prime} \in V_G$,
\begin{equation}\label{maxconsensus}
\mathbf{b}_i(t) = \mathbf{b}_{i^{\prime}}(t) = \max\{  \mathbf{b}_1(0), \ldots, \mathbf{b}_{|V_G|}(0) \},
\end{equation}
where ${\rm max\{\cdot\}}$ is the component-wise  maximum.
\end{definition}

%
 \noindent
{\bf Assumptions:} we assume that physical nodes are aware of the physical outgoing link capacity to reach each of its first-hop neighbors to propagate the highest bids, and the routing table for the path embedding phase
%, and the diameter $D$ of the physical network,  useful as a termination condition: if a physical node has received more than $D$ messages the auction phase terminates.~\footnote{Algorithms to compute the diameter of a network in a distributed way are well known~\cite{consensusBook}, and they are outside the scope of this paper.}


   \begin{figure}[t]
\begin{center}
    \includegraphics[scale=0.25]{overview.pdf}
\end{center}
\caption{(a) Virtual network with capacity constraints to be embedded. (b) Each physical node (PN) can be owned by  a different InP, and can have a different capacity. (c) CAD workflow: a virtual link embedding phase follows the virtual node bidding and agreement phases.}
\label{fig:VNexample}
\end{figure}



==> vne-model2.tex <==
%\textcolor{red}{FLAVIO: Can you include pieces of code in the text and explain them, as opposed to have one big figure with all the code at the end?}

%In previous section we described the basic concepts of Alloy modeling language. For an abstract enough system, Alloy is a helpful and easy to use language to model the system.
In this section we overview our max-consensus distributed auction Alloy model, applied to the context of a virtual network mapping protocol  (see Section~\ref{sec:applications}).
%
We separate the model into a static and a dynamic part: the static sub-model refers to the two types of networks, $i.e.$ the underlying hosting physical network, and the virtual network to be mapped with the max-consensus based auction protocol.


\junk{
\begin{figure}
\begin{flushleft}
  {\scriptsize
    \begin{verbatim}
sig pnode{
    pcp: one Int,
    pid: one Int,
    initBids: vnode->Int,
    initBidTimes: vnode->Int,
    pconnections: some pnode
}
%
sig vnode{
    vid: one Int,
    vconnections: set vnode
}
%
fact pcapacity{
    all p: pnode |
    (sum vnode.(p.initBids) ) <= p.pcp
}
%
fact conectivityFact{
    all disj pn1,pn2:pnode |
    ( pn1.pid != pn2.pid) and
    (pn1 in pn2.pconnections <=> pn2 in pn1.pconnections)
}
%
fact selfLoopFact{
    all pn:pnode |
    (pn.pcp) >=0 and (pn.pid) >=0 and
    no (pn & pn.pconnections)
}
%
fact vnodeFact{
    all disj vn1,  vn2: vnode |
    vn1.vid > 0 and vn1.vid != vn2.vid
}
    \end{verbatim}
    }
  \end{flushleft}
  \caption{A part of Alloy model of the physical and virtual network}
  \label{fig:alloy-pnode-vnode}
\end{figure}
%
}


\noindent
{\bf Static Model.} %We now presents a fragment of the static model, explaining how the elements of both the physical  and the virtual network are modeled. %(Figure~\ref{fig:alloy-pnode-vnode}).
%
%
A simplified version of the signature \texttt{pnode} was explained in Section~\ref{sec:alloy}. A more complete version of this signature includes a ternary relation \texttt{initBids}, that models the initial values that an agent (physical node) assigns when bidding on some subset of all virtual nodes.
Another ternary relation \texttt{initBidTimes} models the corresponding time that the physical node has made the bids on the virtual nodes:

%
{\scriptsize
\begin{verbatim}
sig pnode{
    pcp: one Int,
    pid: one Int,
    initBids: vnode->Int,
    initBidTimes: vnode->Int,
    pconnections: some pnode
    p_T: one Int,
    p_U: one utility,
    p_RO: one release_outbid
    ... // add your policy
}
\end{verbatim}
}
%



\junk{
The second signature models the virtual nodes in the network and their connection as a virtual network. The rest
are some of constraints on physical and virtual nodes, modeled as Alloy facts.
Using these facts we can regulates some rules on how our network should behaves and look like.
}

As we described in Section~\ref{sec:applications}, the virtual network mapping problem maps  constrained virtual networks on a constrained physical network, eventually owned by multiple, federated infrastructure providers. Our model captures any constraints in the form of an Alloy {\tt fact}; for example, to impose that physical nodes can bid on virtual nodes only if they  have enough capacity to host them, we define the following fact:

{\scriptsize
\begin{verbatim}
fact pcapacity{
      all p: pnode |
      (sum vnode.(p.initBids) ) <= p.pcp
}
\end{verbatim}
}

By definition, an Alloy relation is modeled with an ordered tuple; this means that unordered relations must be explicit, $e.g$, an undirected link has to be modeled using two (directed) relations, as in our \texttt{pconnectivity} fact:


{\scriptsize
\begin{verbatim}
fact pconnectivity{
     all disj pn1,pn2:pnode |
     (pn1.pid != pn2.pid) and
     (pn1 in pn2.pconnections <=>
     pn2 in pn1.pconnections)
}
\end{verbatim}
}

%%%%%%%%%
Our static model includes several other facts that regulate basic (networking) properties, that we do not report for lack of space. For example, a \texttt{selfLoop} fact is required to avoid that the source and the destination identifiers of a (physical or virtual) link are not identical, or, a \texttt{vnodeFact} set should impose that the identifier of the agent is non-negative, and unique:

{\scriptsize
\begin{verbatim}
fact vnodeFact{
     all disj vn1,  vn2: vnode |
     vn1.vid > 0 and vn1.vid != vn2.vid
}
\end{verbatim}
}

Note that the \texttt{vnodeFact} is in addition to the \texttt{vnode} signature, that defines this actionable item set.

{\scriptsize
\begin{verbatim}
sig vnode{
    vid: one Int,
    vconnections: set vnode
}
\end{verbatim}
}

%Using  the  \texttt{pconnectivity} fact we impose the rule that for every two disjoint physical nodes, their ID has to be different, and their connection, if exist, it is undirected.

%\texttt{selfLoopFact} takes care of the fact that no self loop exists in a network and finally fact \texttt{vnodeFact} says the ID of all virtual nodes are positive values and unique.

\noindent
{\bf Dynamic Model.} The dynamic behavior of the network is modeled as a \emph{transition system}, and the sequence of state changes is regulated by the consensus-based auction protocol.
%
Such network state updates are captures in our model with the signature
\texttt{netState}.

{\scriptsize
\begin{verbatim}
sig netState {
    bidVectors: some bidVector,
    time: one Int,				
    buffMsgs: set message
}
\end{verbatim}
}
%open util/ordering[netState]

The states of the (physical) network of agent (physical nodes) is updated as (bid) messages are exchanged among physical nodes.
%
The signature \texttt{netState} captures such views for all
agents (physical nodes) through a {\tt bidVectors} relations, that contains the current view of each agent, $i.e.$, the vectors ${\bf a}$, ${\bf b}$, ${\bf t}$, and ${\bf m}$ (see Figure~\ref{example}).
%
The relation {\tt time} models the time of each network state.
%

The set of unprocessed messages are modeled with a buffer \texttt{buffMsgs} binary relation. This relation captures the correspondence between states and messages in transit.
%
%Using a library module \texttt{util/ordering} we define instances of network's states as an ordered chain.

{\scriptsize
\begin{verbatim}
sig message{
    msgSender: one pnode,
    msgReceiver: one pnode,
    msgWinners: vnode->(pnode + NULL),
    msgBids: vnode->Int,
    msgBidTimes: vnode->Int
}
\end{verbatim}
}

Aside from information about sender and receiver, each \texttt{message} signature contains the view of the sender agent about the states required to reach a max-consensus on the actionable items (virtual nodes). Such states are modeled by three ternary relations: the bid vector \texttt{msgBids}, the time-stamp vector  \texttt{msgBidTimes}, and the allocation vector \texttt{msgWinners}. Note how, after a message is being processed, these relations are used to update the {\tt bidVectors} states: ${\bf a}$, ${\bf b}$, ${\bf t}$, and the bundle vector ${\bf m}$ for each physical node, for a distributed winner determination (see Figure~\ref{example}).



%Besides, \texttt{netState} also contains the binary relation \texttt{buffMsgs} which models all messages awaiting to reach their destination.
%Signature \texttt{message} models a message that is sent from a the physical node \texttt{msgSender} to the receiver \texttt{msgReceiver}.


%
%
\junk{
\begin{figure}
\begin{flushleft}
  {\scriptsize
    \begin{verbatim}
sig netState {
    bidVectors: some bidVector,
    time: one Int,
    buffMsgs: set message
}
%
open util/ordering[netState]
%
sig bidVector{
    bvPn:one pnode,
    winners: vnode->(pnode + NULL),
    winnerBids: vnode->Int,
    bidTimes: vnode->Int,
    excludedVN: set vnode
}
%
sig message{
    mSender: one pnode,
    mReceiver: one pnode,
    mWinners: vnode->(pnode + NULL),
    msgWinnerBids: vnode->Int,
    msgBidTimes: vnode->Int
}
%
fact messagingFact{
    all s: netState, s': s.next | one m:message |
    messaging[s, s', m]
}
%
pred messaging(s, s': netState, m:message){
    s'.time > s.time and
    (s.buffMsgs - s'.buffMsgs) = m and
    ((one v:vnode |
        outBid[s, v, m] and
        updateAndRebid[s, s', v, m])
    or
    ((no v:vnode | outBid[s, v, m]) and
        checkAllOfVnodes[s, s', m]))	
}
    \end{verbatim}
    }
  \end{flushleft}
  \caption{A part of the model of messaging and state transition in a network based on VNE protocol.}
  \label{fig:alloy-state-message}
\end{figure}
%Figure \ref{fig:alloy-state-message} shows a fragment of the model that covers the messaging and state transition in our Alloy model.
}
%
%
%Keyword \texttt{first} points to the first state while \texttt{first} points to the last one.
%
%
%The view of each physical node is modeled by signature \texttt{bidVector}. Each \texttt{bidVector} is related to exactly one physical node by relation \texttt{bvPn}, and it keeps the track of the bidding (winner, value and time).
%
%for each virtual node using ternary relations \texttt{winners}, \texttt{winnerBids} and \texttt{bidTimes} respectively.
%Formally speaking, in any instance of our model, for every physical network at every network state, exists an instance of signature \texttt{bidVector} that shows the three vectors ``bid vector", ``assignment vector" and ``bid time vector".




The core of the consensus-based auction protocol is modeled by some {\it constraint paragraphs}, that capture the behavior of the agents, their state transitions and message processing.
In particular, the Alloy fact {\tt stateTransition} models that messages are being process in sequence, from state $s$ to $s^{\prime}$:

{\scriptsize
    \begin{verbatim}
fact stateTransition{
     all s: netState, s': s.next | one m:message |
     messageProcessing[s, s', m]
}
\end{verbatim}
}
%

%


%The important ones are the fact \texttt{messagingFact} and the predicate \texttt{messaging}. The fact \texttt{messagingFact} says that for each two consecutive states, exactly one floating message is processed.

%Modeled by \texttt{messaging} predicate, this message processing regulates how the state of network changes from one to the next based on VNE protocol.
\junk{% add in the TR after ICNP review
The auxiliary predicate and facts are omitted but interested readers can refer to the appendix for more details.
}

%
%
%
\section{Using Alloy to Analyze MCA Convergence}\label{sec:property-checking}

%Model checking is used to verify property of a protocol.
Our model enables us to study the convergence  properties of the MCA protocol. We first introduce the assertion for checking this property, and then we show how specific combinations of the MCA policy instantiations may or may not lead to convergence of the MCA protocol.

 %The MCA protocol should reach an agreement on the winner actionable items.
%
Checking the convergence property in Alloy means checking weather or not the consensus assertion holds. All the agents (physical nodes) need to agree on the view of two vectors (Definition~\ref{def:maxConsensus}): ($i$) the assignment vector,
which represents the winner of the actionable items ($e.g.$ virtual nodes), ($ii$) and the bid vector.
The assertion consensus is coded in Alloy as follows:

%
{\scriptsize
\begin{verbatim}
    assert consensus{
	     (#(netState) >= val) implies consensusPred[]
    }
    pred consensusPred{
        some s: netState
        | all disj bv1,bv2: s.bidVectors |
        (
            (bv1.winners    = bv2.winners) and
            (bv1.winnerBids = bv2.winnerBids)
        )
    }
\end{verbatim}
}
%

%%%% call the policy
%%% show the code
%%% explain why it does not converges.


%%%%
%
We assert the consensus property over several scopes, without finding a counter-example of non-convergence, which means that the assertion holds for the tested scope.

%
Bounds on convergence time of the  consensus-based auction protocol described have been found in both cloud computing~\cite{CADpaper} and robotic network~\cite{cbba}. In particular,  the number of messages required to reach consensus is upper bounded by the size of the actionable item set times the diameter of the network of agents (in number of hops). Intuitively, this is because the maximum bid for each item ($e.g.$, virtual node), only has to traverse the network of agents once. This bound was used to set our val parameter in the consensus assertion.

%\ref{rm:overbid}
% motivate need for proper checking

We tested the same consensus property under circumstances of protocol misbehavior or misconfiguration. For example, we removed from our model the necessary condition discussed in Remark~(\ref{rm:overbid}), allowing physical nodes to re-bid after they were outbid on a virtual node, and we found counter-examples as expected. %Moreover, counterexample is output  for show the details of the
%
A consequence of the existence of such counter example is that the protocol is not resilient to {\it rebidding attacks}.
%
%An interesting research question  ...
%A single agents may cause failure or instability by  the network to reach an agreement from malicious agents. One

%The question is does the system finally reaches consensus if some nodes behave differently.
% To check this property we embed in our model the the ability that nodes can do rebidding in case they got overbid by some other node.
%Checking the assertion \texttt{consensus} under the new conditions, Alloy  Analyzer showed that there are scenarios that the network will never reach general consensus.

%There are scenarios that for some specific network, there is repeating cycle in state transition run of the network. Unfortunately the found counterexample is huge and complicated and does not fit in this report.






==> vne.tex <==
%What is the VN embedding and who cares
Describe the protocol here, the challenges (NP-hard) of distributing a problem that is NP-hard\\

%Why consensus based?
Describe the guarantees found in earlier work\\

%Describe the work in the context of this paper and why it's important to have an alloy model
State our optimistic assumptions and explain: \\
1. we may have skipped some corner case in our testing that alloy would find. \\
2. Every pnode follows the asynchronous conflict resolution rules. \footnote{We should have a technical report with the final working version of the table in the appendix, not to include in the final paper}\\
3. Pnode do not overbid  \\
4. Admit that the protocol is vulnerable to attack and pose research question. Mention also that second price auctions may not work here, because they don't maximize the revenue of the auctioneer. Also, path auctions [cite Frugal Path Auction of Tardos] assume always a second path, but if you are the only pnode to the destination you can bid as much as you want there is no way to enforce truthfulness. Explain that this is not a problem, as in BGP  happens the same thing, and provider find commercial agreements.

